The One-Sided Isometric Extension Problem

Let $\Sigma$ be a codimension one submanifold of an $n$-dimensional Riemannian manifold $M$, $n\geqslant 2$. We give a necessary condition for an isometric immersion of $\Sigma$ into $\mathbb R^q$ equipped with the standard Euclidean metric, $q\geqslant n+1$, to be locally isometrically $C^1$-extendable to $M$. Even if this condition is not met, "one-sided" isometric $C^1$-extensions may exist and turn out to satisfy a $C^0$-dense parametric $h$-principle in the sense of Gromov.

==> chart.tex <==
\psfrag{M}{$M$}
\psfrag{U}{$U$}
\psfrag{H}{$\Sigma$}
\psfrag{p}{}
\psfrag{O}{$\bar\Omega$}
\psfrag{B}{$B$}

==> codim21.tex <==
\psfrag{r}{$S^1_{r_2}(-1)$}
\psfrag{s}{$S^2_{r_1}(0)$}


==> corr.tex <==
\psfrag{m}{$\mu$}
\psfrag{n}{$-\mu$}
\psfrag{f}{$f$}


==> cutoff.tex <==
\psfrag{j}{$j$}
\psfrag{O}{$\overline{\Omega_j^c}$}
\psfrag{P}{$\bar\Omega_j$}

==> homotopy.tex <==
\psfrag{a}{$u_1$}
\psfrag{b}{$u_2$}
\psfrag{c}{$\vdots$}
\psfrag{d}{$\tfrac{1}{2}$}
\psfrag{e}{$\tfrac{3}{4}\ldots 1-\tfrac{1}{2^n}$}
\psfrag{h}{$u_0$}

